Advancing Chart Question Answering with Robust Chart Component Recognition

Chart comprehension presents significant challenges for machine learning models due to the diverse and intricate shapes of charts. Existing multimodal methods often overlook these visual features or fail to integrate them effectively for chart question answering (ChartQA). To address this, we introduce Chartformer, a unified framework that enhances chart component recognition by accurately identifying and classifying components such as bars, lines, pies, titles, legends, and axes. Additionally, we propose a novel Question-guided Deformable Co-Attention (QDCAt) mechanism, which fuses chart features encoded by Chartformer with the given question, leveraging the question's guidance to ground the correct answer. Extensive experiments demonstrate that the proposed approaches significantly outperform baseline models in chart component recognition and ChartQA tasks, achieving improvements of 3.2% in mAP and 15.4% in accuracy, respectively. These results underscore the robustness of our solution for detailed visual data interpretation across various applications.

==> latex/3methods.tex <==
\section{Methods}
\subsection{Task Formulation}
\paragraph{Chart Component Recognition}
Given an input chart image \(I\) with dimensions \(H \times W\), the task of chart component recognition is to identify and classify various components within the chart. These include both graphical and textual elements, such as lines, bars, legends, and chart titles. Let $C$ be the set of all chart component types, e.g., $C = \{\text{"Bar"}, \text{"Line"}, \text{"Pie"}, \ldots\}$. Let \(M_c\) represent the set of instance segmentation regions corresponding to a particular chart component type \(c \in C\), and $M = \{ M_c \}_{c \in C}$ be the set of all annotations for the image $I$. 
The objective is to design and train a model that learns to accurately identify and classify each chart component in unseen chart images as shown in Figure \ref{fig:ccr}. 


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/chart-chart_element.pdf}
    \caption{The chart component recognition task}
    \label{fig:ccr}
\end{figure}

\paragraph{Chart Question Answering}

Given an input image $I$ and natural language question $Q$, the task of chart question answering is to provide a correct answer $A$.


\subsection{\texorpdfstring{\!}{}Question-guided Deformable Co-Attention}

This section introduces Question-guided Deformable Co-Attention (\textbf{QDCAt}).
Its purpose is twofold: to fuse image features from complimentary encoders, and to incorporate information guided by the question.
The main components of QDCAt are a question-guided offset network and a deformable co-attention block.

\subsubsection{Question-guided Offset Network}\label{sec:qgoff}
A Vision Question Answering (VQA) model requires the ability to capture complex spatial relationships and patterns in images and associate them with questions. To learn dynamic, question-sensitive keys and values conditioned on the queries, we employ \emph{deformable sampling} in the \Model{} backbone and introduce a novel \emph{question-guided deformable sampling} in \Modelvqa{} for the ChartQA task. \emph{Deformable sampling}, a procedure introduced in \cite{xia_dat_2023} involves processing input through an offset network $\theta_\text{offset}$ to compute offsets $\Delta p$, then sampling said input at offset locations $p + \Delta p$.
The overall structure of $\theta_\text{offset}$ remains similar to that in \cite{xia_dat_2023}, consisting of the following.
\begin{itemize}
    \item \textbf{Convolution Layer:} Pass the input features through a \( k \times k \) convolution layer.
    \item \textbf{Normalization and Activation:} Apply Layer Normalization and GELU activation to the convolved features.
    \item \textbf{Projection Layer:} Pass the activated features through a \( 1 \times 1 \) convolution layer with $2$ output channels to predict the 2-D offset values.
\end{itemize}
The proposed Question-guided offset network is distinct in being conditioned on the question embedding provided in the ChartQA task, as seen in Figure~\ref{fig:chartqa_model}.
We obtain the token embeddings of the question as provided by MBart \cite{liu_multilingual_2020} (without backpropagation), then linearly interpolate to the maximum token length and denote the output as $z$.
The input tensor $x$ is passed through a projection layer\footnote{We use the term 'projection layer' to refer to a convolution layer with a $1 \times 1$ kernel.} parametrized by the weights $W_a$ to obtain $a = x W_a$.
This matches the channel dimension of the two modes of input, allowing us to take the dot product of $z$ and $a$ to get $z a^\top$, which we feed into the offset network,
$$ \Delta p = \theta_\text{offset}(z a^\top), \quad \tilde{x} = \phi(x; R ( p + \Delta p ))\ .$$
The features \( \tilde{x} \) are sampled with bilinear interpolation at the learned region \( R \) of the deformed points \( p + \Delta p \). The idea behind giving the offset network the combined input of $z$ and $a$ is to make the sampled points $p + \Delta p$ align with image locations with semantic significance for the question of the particular data sample, as opposed to locations with overall significance. This allows further features learned by the model to represent visual queues with specific relevance to the given question.
A visual representation of the question-guided offset network is provided in Figure~\ref{fig:qgoff} in Appendix~\ref{sec:appendix}.

\subsubsection{Deformable Co-Attention Block}


When incorporating additional information into an existing model or integrating features from various modalities, it is essential to preserve prior knowledge while progressively assimilating new information. We introduce the deformable co-attention block, a module that incorporates both deformable sampling and multiple feature sources. Similar to standard attention modules, we obtain query, key, and value vectors through projections of the input. The \textit{self-attention} module is summarized as follows
\begin{align*}
    q = x W_q\ , \quad k = x W_k\ , \quad v = x W_v\ ,\\
    \text{Attention}(q, k, v) = \text{softmax} \left( q k^\top / \sqrt{d} \right) v\ ,
\end{align*}
with $x$ denoting the input features.
To emphasize attention computed at semantically relevant features, \emph{deformable attention} \cite{xia_dat_2023} computes the key and value vectors from features $\tilde{x}$ obtained via deformable sampling. The input projections are
\begin{align*}
    q = x W_q\ , \quad k = \tilde{x} W_k\ , \quad v = \tilde{x} W_v\ ,\\
    \Delta p = \theta_\text{offset}(q), \quad \tilde{x} = \phi(x; R ( p + \Delta p ))\ .
\end{align*}
The projection $q$ of the image features guides the movement of deformable points, and attention is computed at the updated locations.
\emph{Co-attention} combines features extracted from multiple modalities. For instance, query vectors are sourced from a language model or audio model, while key and value vectors are derived from a vision model.

The proposed \emph{deformable co-attention} utilizes this approach to combine features from multiple backbones, denoted by $\tilde{x}$ and $y$.
The former is guided by language features via an offset network. %as described in Section~\ref{sec:qgoff}.

The projections are applied as follows:
\begin{align*}
    q = y W_q\ , \quad k = \tilde{x} W_k\ , \quad v = \tilde{x} W_v\ ,\\
    \text{DCAttention}(q, k, v) = \text{softmax} \left( q k^\top / \sqrt{d} \right) v\ .
\end{align*}


We use $x$ and $y$ to denote the two input features of the deformable co-attention block.
In practice, these features are produced by complementary visual backbones, the former using deformable attention and the latter self-attention.
As described in Section~\ref{sec:qgoff}, a combination of visual and language features is then passed through an offset network to compute offsets $\Delta p$, and after bilinear sampling at the deformed points we obtain $\tilde{x}$.
These sampled features are used to obtain $k$ and $v$, while $q$ is projected from $y$.
Following standard practices, we combine $q$ with $k$, scale by the square root of the dimension $d$, apply softmax, and combine with $v$.



In the deformable co-attention block, the outputs of the above steps are passed through residual connections, normalization layers, and a feed-forward network. The Add and LayerNorm operations perform element-wise addition of features. Their first occurrence adds the features from the original vision transformer encoder, denoted as $y$, and the features processed by \emph{deformable co-attention}.
$$ b = \text{LayerNorm}(y + \text{DCAttention}(q, k, v))\ .$$
The feed-forward network consists of a $3 \times 3$ convolution layer followed by ReLU activation. The second occurrence of Add and LayerNorm adds the previous occurrence output $b$ with the output of the feed-forward network. These steps are summarized as follows:
\begin{align*}
    \text{FFN}(b) &= \text{ReLU} ( \text{CNN}(b) )\ ,\\
    c &= \text{LayerNorm}(b + \text{FFN}(b))\ .
\end{align*}



The output $c$ is lastly projected via $W_o$ to obtain $o = c W_o$, which is the output of the deformable co-attention block as the final image feature.


\subsection{Model Architecture}

\subsubsection{\Model{}}\label{sec:chartformer}
The \Model{} model consists of three main modules: a vision backbone, a pixel decoder, and a mask transformer decoder. The model pipeline is illustrated in Figure \ref{fig:chart_model}.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/chart.drawio.pdf}
    \caption{The \Model{} model structure}
    \label{fig:chart_model}
\end{figure*}

In the development of \Model{}, we adopt the detection pipeline from Mask2Former \cite{cheng_masked-attention_2022}, integrating it with DAT \cite{xia_dat_2023} as the backbone.  
We employ a transformer encoder-decoder structure, with the backbone model serving as the encoder. The input chart image $I_{H \times W}$  undergoes processing by a CNN layer to generate an initial feature map $E_{512 \times H \times W}$ with a channel size of 512. This feature map is fed into the backbone network for further processing and feature learning. The encoder extracts features (denoted as $ f $) from the input image $ I $, which are then passed to a pixel decoder. The pixel decoder upsamples the extracted features $ f $ and outputs a 2D per-pixel embedding $P_{C \times H \times W}$. Subsequently, a Mask2Former \cite{cheng_masked-attention_2022} decoder takes both the object query and the pixel embedding as input and predicts a mask embedding vector $M_{C \times N}$, where $ N $ represents the number of object queries. Finally, the dot product of $ P $ and $ M $ results in an independent per-pixel mask $O_{H \times W \times N}$. 

\paragraph{Visual Backbone}


In the context of the \Model{} backbone, which builds upon the Vision Transformer, the architecture follows the established four-stage setup. However, each stage in \Model{} is enriched with two distinct attention blocks: neighborhood attention blocks \cite{hassani_neighborhood_2022} and deformable attention blocks \cite{xia_dat_2023}. These specialized attention mechanisms allow \Model{} to capture both local and global contextual information effectively, thereby enhancing the ability to extract meaningful features from chart images. \zoe{gonna add detailed parameters in appendix}


\subsubsection{\Modelvqa{}} The model consists of three main modules: two transformer vision encoders, a Question-guided Deformable Co-Attention (QDCAt) fusion block that fuses the output of two encoders, and a text decoder as shown in Fig \ref{fig:chartqa_model}.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figs/chart-chartformer.drawio.pdf}
    \caption{The \Modelvqa{} model structure}
    \label{fig:chartqa_model}
\end{figure*}

\paragraph{\Model{} Encoder}
We include the backbone of the \Model{} model as a secondary image encoder, utilized to capture explicit chart segment information. This secondary encoder is structured as described in the "Visual Backbone" paragraph of Section~\ref{sec:chartformer}. During the fine-tuning stage on the ChartQA dataset, we freeze the weights of the \Model{} model to reduce training costs. By leveraging the \Model{} backbone as a supplementary encoder, the model gains access to richer visual information, enhancing its performance in ChartQA tasks.

\paragraph{Transformer Vision Encoder}
Donut \cite{kim_ocr-free_2022} is pretrained on a large dataset using a pseudo-OCR task focused on receipts understanding and parsing. To optimize computational and memory efficiency, we opt not to pretrain a new vision encoder-decoder model, and instead add richer visual and text information using the \Model{} encoder and question-guided deformable co-attention.



\paragraph{Text Decoder}
Following the approach of Donut \cite{kim_ocr-free_2022}, we also employ the MBart decoder \cite{liu_multilingual_2020} for answer output generation. Task-specific prompts, for instance, \texttt{<chartvqa>}, \texttt{<s\_answer>} are provided to the decoder as special tokens, and the decoder generates the output by predicting the next token based on the prompted context.

